Methodologies for Quantifying (Re-)randomization Security and Timing under JIT-ROP

Just-in-time return-oriented programming (JIT-ROP) allows one to dynamically discover instruction pages and launch code reuse attacks, effectively bypassing most fine-grained address space layout randomization (ASLR) protection. However, in-depth questions regarding the impact of code (re-)randomization on code reuse attacks have not been studied. For example, how would one compute the re-randomization interval effectively by considering the speed of gadget convergence to defeat JIT-ROP attacks?; how do starting pointers in JIT-ROP impact gadget availability and gadget convergence time?; what impact do fine-grained code randomizations have on the Turing-complete expressive power of JIT-ROP payloads? We conduct a comprehensive measurement study on the effectiveness of fine-grained code randomization schemes, with 5 tools, 20 applications including 6 browsers, 1 browser engine, and 25 dynamic libraries. We provide methodologies to measure JIT-ROP gadget availability, quality, and their Turing-complete expressiveness, as well as to empirically determine the upper bound of re-randomization intervals in re-randomization schemes using the Turing-complete (TC), priority, MOV TC, and payload gadget sets. Experiments show that the upper bound ranges from 1.5 to 3.5 seconds in our tested applications. Besides, our results show that locations of leaked pointers used in JIT-ROP attacks have no impacts on gadget availability, but have an impact on how fast attackers find gadgets. Our results also show that instruction-level single-round randomization thwarts current gadget finding techniques under the JIT-ROP threat model.

==> sections/12-availability.tex <==
%-------------------------------------------------------------------------------
%\section*{Availability}
%-------------------------------------------------------------------------------

%USENIX program committees give extra points to submissions that are backed by artifacts that are publicly available. If you made your code or data available, it's worth mentioning this fact in a dedicated section.

%-------------------------------------------------------------------------------

==> sections/todos.tex <==
\section{ToDos}

\subsection{Meeting discussions}
\begin{itemize}
    \item Explain the conventional metrics are not enough for demonstrating effectiveness of fine-grained of ASLR
    \item Limitations of entropy metrics
    \item Why aslr measurement is needed with citations
    \item A name is needed for our tool
    \item Explain the leave issue with gadget chain
    \item explain the alternatives of register corruption rate techniques
\end{itemize}

\subsection{Additionals}
\begin{itemize}
    \item New experiments by setting different limits on gadget length
    \item Experimenting and measuring gadgets by setting different parameters in multicompiler
    \item Design experiments to use RUNTIMEASLR
    \item Experimenting more applications and dynamic libraries
    \item Need source code for Oxymoron 
\end{itemize}

\subsection{New additions}

\begin{enumerate}
\item *Incorporation of instruction and register randomization tools (e.g., multi-compiler and ILR).
\item *Incorporation of at least 15 applications and 20 libraries including Tor and other browsers
\item *Average over multiple runs. We can show mean and variation in tables, or error bars in figures.
\item *Performing 1-2 traditional ASLR effectiveness measurements, like entropy. What’s the most popular metric for ASLR?
\item Inclusion of other attack actions such as reading user data or cookies other than just issuing system calls
\item Inclusion of other evaluation metrics: the amount of work (e.g., repeated exploitation attempts, or repeated pointer leaks, or duration/length of memory travels/scans) needed to discover the gadgets in the randomized layout.

\end{enumerate}


\subsection{Analysis}
\begin{enumerate}
\item *why does selfrando introduce leave instructions?
\item What is the difference between leaking a code pointer and leaking a stack/heap/data pointer regarding the reachability of ROP gadgets?
\item *why does the register corruption rate increase?
\item *why do randomization tools increase the number of gadgets for some gadget types?
\item *Where do the libc pointers found on the stack and the heap point (e.g., to which function they point, in which data structure they occurred, ...)?
\end{enumerate}


\subsection{Clarifications}
\begin{enumerate}
\item Adding a Venn diagram of all these gadget types
\item Clarifying the problem associated with linux-vdso.so, libpthread.so, libdl.so, libm.so, or libpcre.so libraries 
\item Clarifying the contradictions [70] by stating that all leaked pointers are equally useful.
\item Adding some description mentioning of zombie gadgets (may not need experiments)
\item Fixing Figure 1: when printed in grayscale, it is not clear what the "blue box" is.
\item Presenting a rough overview of the complexity of finding gadgets
\item Adding a paragraph describing what a Turing-complete set of gadgets looks like
\item Clarifying this inside the text (since the layouts change after each application of randomization, it would be useful to analyze multiple instances of the same application and to average the counted gadgets across them)
\end{enumerate}

==> sections/z-bk-04-jit-vs-basic-rop.tex <==
%------------------------------------------------------------------------------------
\section{JIT-ROP vs. Basic ROP Attacks}\label{attack-workflow}
%CCS20% \section{Comparison of JIT-ROP and Basic ROP Attacks}\label{attack-workflow}
%------------------------------------------------------------------------------------
\noindent We manually analyze a number of advanced attacks to extract common attack elements and identify unique requirements. We illustrate the key technical differences between JIT-ROP and conventional (or basic) ROP attacks. This section helps one understand our experimental design in Section~\ref{exp-design} and findings in Section~\ref{exp_eval}. We analyze various attack demonstrations with a focus on attacks (e.g., \cite{davi2015isomeron, snow2013just, bittau2014hacking, carlini2014rop}) in our threat model. 

%backes2014oxymoron, maisuradze2016cannot, carlini2015control, goktas2014out, hu2016data



%\onecolumn
\begin{figure}[!tbph]
  \centering
  %,natwidth=610,natheight=642
  \includegraphics[width=0.48\textwidth]{figures/attack-workflow-new7.png}
  \caption{An illustration of the commonalities and differences between a conventional (or basic) ROP attack (bottom) and a JIT-ROP attack (top). The top gray-box highlights the key steps in JIT-ROP to overcome fine-grained ASLR.}
  \label{fig-attack-tree}
\end{figure}
%\twocolumn




To overcome both coarse- and fine-grained ASLR and conduct an attack to gain privileged operations, an attacker needs to perform the tasks presented in Figure \ref{fig-attack-tree}.  The attack workflow has three major components: \textbf{\textit{memory layout derandomization}}, \textbf{\textit{system access}}, and \textbf{\textit{payload generation}}. We describe each component in Sections~\ref{workflow-memory-derand}, \ref{workflow-system-access}, and \ref{workflow-payload-gen}, respectively.

\begin{itemize}

\item {\em Memory layout derandomization}: Due to the W$\oplus$X defense, attackers must reuse code (via gadgets) in their attacks. Attackers need to derandomize the memory layout to discover gadgets (steps \circled{2}-\circled{4} for JIT-ROP and steps \circled{2$'$} and \circled{4$'$} for basic ROP in Figure \ref{fig-attack-tree}). Usually, attackers leverage memory corruption vulnerabilities to leak memory \cite{strackx2009breaking} and start the derandomization process utilizing the leaked memory.

\item {\em System access}: Attackers invoke system APIs or gadgets for carrying out practical tasks \cite{bletsch2011jump, bittau2014hacking, snow2013just, carlini2014rop, davi2015isomeron}. However, some attack scenarios may not require system calls. In this paper, we focus only those attacks that utilize system calls. 
%Attackers invoke system calls through \verb1syscall1 gadgets. 
One can find {\em syscall} gadgets through step \circled{4} in JIT-ROP along with other gadgets. In basic ROP, one must find the {\em syscall} gadgets through pointer leakage in system libraries (like {\em libc}) or application binaries (step \circled{9}).

%\item {\em System access}: Attackers access privileged system operations by issuing system APIs or gadgets. However, useful attacker actions may also include reading user data (such as email) or stealing authentication tokens (like cookies). These actions do not involve system calls. In this paper, we only consider those attacks that utilize system calls. Attackers invoke system calls through \verb1syscall1 gadgets. One can find \verb1syscall1 gadgets through step \circled{4} in JIT-ROP along with other gadgets. In basic ROP, one must find the \verb1syscall1 gadgets through pointer leakage in system libraries (like \verb1libc1) or application binaries (step \circled{9}).

%\item {\em System access}: Attackers need to issue system APIs or gadgets to perform privileged operations. However, accessing system APIs is difficult because of ASLR. In addition, a level of indirection (e.g., \textbf{G}lobal \textbf{O}ffset \textbf{T}able (GOT) in Linux, \textbf{I}mport \textbf{A}ddress \textbf{T}able (IAT) in Windows, and RaTTle \cite{backes2014oxymoron} in custom implementations) protects the access. As a result, an attacker needs to follow some techniques to access the system functions or gadgets. One can find system gadgets through step \circled{4} in JIT-ROP.

%\gtan{Why step \circled{4} is in both "memory layout derandomization" and "system API access"?}

\item {\em Payload generation}: Attackers generate payloads by putting many pieces (e.g., gadgets, functions, constants, strings, etc.) together. This process must ensure a setup for calling system functions or system gadgets. Steps \circled{5} and \circled{5$'$} in Figure~\ref{fig-attack-tree} correspond to the payload generation operation for JIT-ROP and basic-ROP, respectively. The target of a payload is to achieve an attack goal, e.g., memory leak, launching a malicious application, or launching a root shell. 

\end{itemize}

%Daphne commented below out
%Each of the three attack components (i.e., \textit{memory layout randomization}, \textit{system API access}, and \textit{payload generation}) has several tasks. In \S \ref{exp_eval}, we experimentally evaluate the important aspects of these three attack components. In the next three sections, we describe the details of each component.



%------------------------------------------------------------------------
\subsection{Memory Layout Derandomization} \label{workflow-memory-derand}
%------------------------------------------------------------------------
\noindent Derandomizing the fine-grained address space layout is the key for mounting code-reuse attacks with gadgets. This step requires overcoming several obstacles.



%-----------------------------------------------------------------------------------
\noindent
\textbf{Memory disclosure}.
\label{workflow-memory-derand-disclosure}
%-----------------------------------------------------------------------------------
The most common way of derandomizing memory layout is through a memory disclosure vulnerability in an application. Attackers use vulnerabilities in an application's memory (e.g., heap overflows, use-after-free, type confusion, etc.) and weaknesses in system internals (e.g., vulnerabilities in the glibc malloc implementation or its variants \cite{argyroudis2012exploiting, heelan2018automatic}, Heap Feng Shui \cite{sotirov2007heap}, Flip Feng Shui \cite{razavi2016flip}) to leak memory contents (Steps \circled{2} and \circled{2$'$}). Details on memory corruption model can be found in \cite{szekeres2013sok, gens2018k} and an example in \cite{strackx2009breaking}.



%------------------------------------------------------
\noindent
\textbf{Code reuse}. \label{code-reuse}
%-----------------------------------------------------
Due to W$\oplus$X defense, adversaries cannot inject code in their payload. ROP~\cite{shacham2007geometry} and its variants Jump-Oriented Programming (JOP) \cite{bletsch2011jump} and Call-Oriented Programming (COP) \cite{goktas2014out} can defeat this defense. These techniques use short instruction sequences (i.e., gadget) from the code segments of a process' address space and allow an adversary to perform arbitrary computations.  ROP tutorials can be found in \cite{snow2013just, davi2011ropdefender}. The difference between basic ROP~\cite{shacham2007geometry} and JIT-ROP~\cite{snow2013just} is described next.

\noindent
{\bf Basic ROP}. Coarse-grained ASLR only randomizes the base addresses of various segments and modules of a process. The content of the segments and modules remains unchanged. Thus, it is feasible for an adversary to launch a basic ROP attack~\cite{basic-rop} using gadgets given a leaked address from the code segment of interest. The adversary only needs to adjust the addresses of pre-computed gadgets w.r.t. the leaked address. Step \circled{4$'$} in Figure \ref{fig-attack-tree} is about this task.

\noindent
{\bf Just-in-time ROP}. Fine-grained ASLR randomizes the base addresses, as well as the internal structures of various segments and modules of a process. Thus, simply adjusting the addresses of pre-computed gadgets (as in the basic ROP) no longer works. An adversary needs to find gadgets dynamically at the time of an exploit. She may attempt to scan the process address space starting from a disclosed code pointer to search for gadgets. However, this linear scanning may lead to a segmentation fault and crash the process due to reading an unmapped memory address. A powerful technique introduced by JIT-ROP~\cite{snow2013just} is code page harvest, which is explained next.
%Adversaries also need techniques to identify the kind of a gadgets while searching for gadgets. This technique can also be applicable in the presence of coarse-grained randomization, but not necessary. 

JIT-ROP attacks exploit the connectivity of code in memory to derandomize and locate instructions. The {\bf code harvest process} in JIT-ROP identifies gadgets at runtime by reading and disassembling the text segment of a process. This process starts with computing the page number of a disclosed code pointer at runtime. A 64-bit system uses the first 52 bits for page numbers if the page size is 4K. Once the page number is computed, the process reads the entire 4K data of that page. A light-weight disassembler converts the page data into instructions. The code harvest process searches for chain instructions, such as {\em call} or {\em jmp} instructions to find pointers to other code pages. 

An illustration is shown in Figure \ref{cp-jitrop}. The code harvest process starts from the disclosed pointer (0x11F95C4), reads 4K page data (0x11F9000-0x11F9FFF), disassembles the data, searches for {\em call} and {\em jmp} instructions to find other pointers (0x11FB410 and 0x11FCFF4) to jump to those code pages. This process is recursive and stops when all the reachable code pages are discovered. We implemented this code harvesting method for our evaluation. It is important to mention that indirect calls to library functions can also be resolved to jump to the library code pages.

%\color{blue}
Snow et. al demonstrated the JIT-ROP attack in a browser. Since exploiting a memory corruption bug remotely covers a wide variety of exploits, a browser could be an ideal interface for JIT-ROP attacks. More specifically, the scripting environment of a browser enables easy interfacing of a JIT-ROP attack payload. The scripting environment, for example, the JavaScript engine allows Just-In-Time compilation which converts JavaScript bytecode to native machine code with the help of the JavaScript virtual machine. That means the scripting environment enables executing dynamically generated code without any concerns related to the DEP or NX memory permission. This way a JIT-ROP JavaScript payload can be executed within a browser. Similarly, JIT-ROP attack payload can be embedded into a PDF reader that supports JavaScript (e.g, Adobe Reader). To launch a JIT-ROP attack in a scripting environment, an attacker must convert any non-scripting code for the scripting environment. For example, the original JIT-ROP framework was written in C/C++ and transpiled the framework to JavaScript to demonstrate an attack on a browser. A framework like Emscripten\footnote{https://emscripten.org} can transpiles C/C++ code to JavaScript/WebAssembly.

%\color{black}


\begin{figure}[!th]
  \centering
  \includegraphics[width=0.45\textwidth]{figures/ch-jitrop7.png}
  \caption{ An illustration of the recursive code harvest process of JIT-ROP~\cite{snow2013just}. An adversary discloses an address from the main executable or libraries (in this case from the main executable) of an application through a vulnerability.
}
  \label{cp-jitrop}
\end{figure}
%\twocolumn



%----------------------------------------------------------------------------------------------------------
\noindent
\textbf{Code page harvest and gadget identification}. \label{workflow-memory-derand-harvest}
%----------------------------------------------------------------------------------------------------------
In step \circled{3} of Figure \ref{fig-attack-tree}, an adversary utilizes the leaked memory address to read code pages of the process' code segments. In step \circled{4}, she can identify and create gadgets by disassembling the read code pages. She can scan for byte values corresponding to {\em ret} opcodes (e.g., 0xC2, 0xC3) and perform a narrow-scoped backward disassembly from there. %She also can use an improved disassembler (e.g., Capstone \cite{capstone-disas}) to perform gadget identification. 
The adversary performs step \circled{3} and \circled{4} repeatedly until she finds enough gadgets for her exploit.




%------------------------------------------------------------
\subsection{System Access} \label{workflow-system-access}
%------------------------------------------------------------
%For meaningful attacks, attackers need to communicate with a system to issue privileged operations, i.e., system calls or system functions. Various mechanisms for accessing system calls or functions depending on the underlying security defenses are described next.

%-----------------------------------------------------------
%\subsubsection{\bf Option 1: Access through system gadgets}:
%-----------------------------------------------------------
%\noindent {\bf Access through system gadgets}: 
\noindent If the execute-only defenses (e.g., XnR\cite{backes2014you}, NEAR\cite{werner2016no}, Readactor\cite{crane2015readactor} and Heisenbyte\cite{tang2015heisenbyte}) and CFI\footnote{which restricts "gadgets" to only legitimately called functions} (e.g., BCFT~\cite{ghaffarinia2019binary}, CCFIR \cite{zhang2013practical} and bin-CFI \cite{zhang2013control}) are not enforced, adversaries do not need to invoke the entire functions to ensure legitimate control flow. An adversary can just chain together enough gadgets for setting up the arguments of a system call and invoking it. This observation is particularly true for Linux, which is the focus of this paper. In Windows exploits~\cite{snow2013just}, the approach is slightly different, as adversaries commonly invoke a system API instead of invoking a system call directly. {\em Syscall} gadgets can be found in an application's code or dynamic library. For basic ROP attacks, attackers can adjust pre-computed system gadgets from dynamic libraries, given that she manages to obtain a code pointer from a dynamic library (e.g., {\em libc}). Step \circled{9} in Figure \ref{fig-attack-tree} is for this task. This task is performed manually and offline. The attacker may obtain the library code pointer from an application's stack or heap or data segment.

%\noindent {\bf Access through system gadgets}: If the execute-only defenses (e.g., XnR\cite{backes2014you}, NEAR\cite{werner2016no}, Readactor\cite{crane2015readactor} and Heisenbyte\cite{tang2015heisenbyte}) and CFI\footnote{which restricts "gadgets" to only legitimately called functions} (e.g., CCFIR \cite{zhang2013practical} and bin-CFI \cite{zhang2013control}) are not enforced, adversaries do not need to invoke the entire functions to ensure legitimate control flow. An adversary can just chain together enough gadgets for setting up the arguments of a system call and invoking it. This observation is particularly true for Linux, which is the focus of this paper. In Windows exploits, the approach is slightly different, as adversaries commonly invoke a system API function instead of invoking a system call directly. Syscall gadgets can be found in the code segment of a process' main executable. The gadgets can also be found in a dynamic library. However, adversaries need a memory leakage from that dynamic library in order to gain access. If an adversary is capable of performing code harvesting from a leaked code pointer, she can access enough system gadgets regardless of the underlying code randomization. 

%If the adversary is not capable of performing code harvesting, she can adjust pre-computed system gadgets from dynamic libraries, given that she manages to obtain a code pointer from a dynamic library (e.g., libc) and the underlying code randomization is coarse grained. Step \circled{9} in Figure \ref{fig-attack-tree} is for this task. This task is performed manually and offline.

%--------------------------------------------------------------------------------------------------------------------------------------------------------------
%\subsubsection{\bf Option 2-4: Access through libc pointers found in an application's stack or heap or data segment}: \label{workflow-system-access-hs-scanner}
%--------------------------------------------------------------------------------------------------------------------------------------------------------------
%\noindent {\bf Access through libc pointers found in an application's stack or heap or data segment}: The heap and stack are the primary sources for information leakage. A stack or heap may contain libc pointers \cite{gil2018hole} that direct attackers to access system gadgets (step \circled{9} in Figure~\ref{fig-attack-tree}).

%\gtan{Why step \circled{9} only appear in basic-ROP in the figure? So JIT-ROP doesn't need to access system API? That would seem strange.}

%-----------------------------------------------------------
\subsection{Payload Generation} \label{workflow-payload-gen}
%-----------------------------------------------------------
\noindent %CCS20%Once an adversary derandomizes the memory layout of a process and gets access to enough gadgets, she glues different parts (e.g., gadgets, functions, strings, constants, etc.) together to build a payload or attack chain. 
Once an adversary gets access to enough gadgets, she constructs a payload or gadget chain with an attack goal in mind. The adversary may generate the payload dynamically at step \circled{5} in the presence of fine-grained code randomization or manually at step \circled{5$'$} in the presence of coarse-grained code randomization and stores the payload in a stack. Because a payload is primarily a set of addresses that point to some existing code in an application's address space, attacks do not execute anything stored in a stack/heap, which is protected by W$\oplus$X. The adversary may utilize the same vulnerability as in step \circled{2} or a different vulnerability to hijack a program's control flow at step \circled{6} to redirect the flow to the stored payload.

It is desirable for attackers to obtain attack chains that have minimal side effects, i.e., having a payload that fulfills attack goals without generating any unnecessary computation. However, this property may not be guaranteed if the gadget availability is limited by code randomization. We refer to the side effect of gadgets as {\em footprints}.  We defined the {\em minimum footprint} gadget and {\em extended footprint} gadget in Section~\ref{threat-model-assumptions}.% and experimentally measure the quality of gadgets in \S\ref{eval-RQ5}.  

For ROP attacks (e.g.,~\cite{carlini2014rop}) that bypass control-flow integrity (CFI) defenses, the attackers also need to prepare specialized payloads in addition to the previous tasks. For example, the Flashing (FS) and Terminal (TM) gadgets in Table~\ref{gadget_type} in the Appendix were designed by Carlini and Wagner~\cite{carlini2014rop} to bypass specific CFI implementations (namely, kBouncer \cite{pappas2013transparent} and ROPecker \cite{cheng2014ropecker}).




